Combining Small-Step and Big-Step Semantics to Verify Loop Optimizations

Verified compilers aim to guarantee that compilation preserves the observable behavior of source programs. While small-step semantics are widely used in such compilers, they are not always the most convenient framework for structural transformations such as loop optimizations. This paper proposes an approach that leverages both small-step and big-step semantics: small-step semantics are used for local transformations, while big-step semantics are employed for structural transformations. An abstract behavioral semantics is introduced as a common interface between the two styles. Coinductive big-step semantics is extended to correctly handle divergence with both finite and infinite traces, bringing it on par with the expressiveness of small-step semantics. This enables the insertion of big-step transformations into the middle of an existing small-step pipeline, thereby fully preserving all top-level semantic preservation theorems. This approach is practically demonstrated in CompCert by implementing and verifying a few new loop optimizations in big-step Cminor, including loop unswitching and, notably, full loop unrolling.

==> pgflibrarybezieroffset.code.tex <==
%% tikz-nfold.sty
%% Copyright 2023 Jonathan Schulz
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3c
% of this license or (at your option) any later version.
% The latest version of this license is in
% http://www.latex-project.org/lppl.txt
% and version 1.3c or later is part of all distributions of LaTeX
% version 2008-05-04 or later.
%
% This work has the LPPL maintenance status 'maintained'.
%
% The Current Maintainer of this work is Jonathan Schulz.
%
% This work consists of the files pgflibrarybezieroffset.code.tex,
% tikzlibrarynfold.code.tex, tikz-nfold-doc.tex, and tikz-nfold-doc.pdf.


% Don't delete this code in case we need it in the future
%
% Split a Bezier curve (de Casteljau's algorithm)
% #1 = time (between 0 and 1)
% #2-#5: control points
% Outputs the first part into \pgf@splitbezier@i@i, ... , \pgf@splitbezier@i@iv,
% and the second part into \pgf@splitbezier@ii@i, ... , \pgf@splitbezier@ii@iv.
%\def\pgf@splitbezier#1#2#3#4#5{%
%  % based on pgfcorepoints.code.tex, \pgfpointcurveattime
%  \edef\pgf@time@s{#1}%
%  \pgf@x=-\pgf@time@s pt%
%  \advance\pgf@x by 1pt%
%  \edef\pgf@time@t{\pgf@sys@tonumber{\pgf@x}}%
%  % P^0_3
%  \pgfextract@process\pgf@splitbezier@ii@iv{#5}%
%  \pgf@xc=\pgf@x%
%  \pgf@yc=\pgf@y%
%  % P^0_2
%  \pgf@process{#4}%
%  \pgf@xb=\pgf@x%
%  \pgf@yb=\pgf@y%
%  % P^0_1
%  \pgf@process{#3}%
%  \pgf@xa=\pgf@x%
%  \pgf@ya=\pgf@y%
%  % P^0_0
%  \pgfextract@process\pgf@splitbezier@i@i{#2}%
%  % First iteration:
%  % P^1_0
%  \pgf@x=\pgf@time@t\pgf@x\advance\pgf@x by\pgf@time@s\pgf@xa%
%  \pgf@y=\pgf@time@t\pgf@y\advance\pgf@y by\pgf@time@s\pgf@ya%
%  \pgfextract@process\pgf@splitbezier@i@ii{}%
%  % P^1_1
%  \pgf@xa=\pgf@time@t\pgf@xa\advance\pgf@xa by\pgf@time@s\pgf@xb%
%  \pgf@ya=\pgf@time@t\pgf@ya\advance\pgf@ya by\pgf@time@s\pgf@yb%
%  % P^1_2
%  \pgf@xb=\pgf@time@t\pgf@xb\advance\pgf@xb by\pgf@time@s\pgf@xc%
%  \pgf@yb=\pgf@time@t\pgf@yb\advance\pgf@yb by\pgf@time@s\pgf@yc%
%  \edef\pgf@splitbezier@ii@iii{\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
%  % P^2_0
%  \pgf@x=\pgf@time@t\pgf@x\advance\pgf@x by\pgf@time@s\pgf@xa%
%  \pgf@y=\pgf@time@t\pgf@y\advance\pgf@y by\pgf@time@s\pgf@ya%
%  \pgfextract@process\pgf@splitbezier@i@iii{}%
%  % P^2_1
%  \pgf@xa=\pgf@time@t\pgf@xa\advance\pgf@xa by\pgf@time@s\pgf@xb%
%  \pgf@ya=\pgf@time@t\pgf@ya\advance\pgf@ya by\pgf@time@s\pgf@yb%
%  \edef\pgf@splitbezier@ii@ii{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
%  % P^3_0
%  \pgf@x=\pgf@time@t\pgf@x\advance\pgf@x by\pgf@time@s\pgf@xa%
%  \pgf@y=\pgf@time@t\pgf@y\advance\pgf@y by\pgf@time@s\pgf@ya%
%  \pgfextract@process\pgf@splitbezier@i@iv{}%
%  \let\pgf@splitbezier@ii@i\pgf@splitbezier@i@iv
%}

% Split the Bezier curve defined by #1-#4 at t=0.5 using de Casteljau's algorithm
\def\pgf@halfsplitbezier#1#2#3#4{%
  % based on pgfcorepoints.code.tex, \pgfpointcurveattime
  % P^0_3
  \pgfextract@process\pgf@splitbezier@ii@iv{#4}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  % P^0_2
  \pgf@process{#3}% removing these does not yield a significant speedup
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  % P^0_1
  \pgf@process{#2}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  % P^0_0
  \pgfextract@process\pgf@splitbezier@i@i{#1}%
  % First iteration:
  % P^1_0
  \pgf@x=.5\pgf@x\advance\pgf@x by.5\pgf@xa%
  \pgf@y=.5\pgf@y\advance\pgf@y by.5\pgf@ya%
  \edef\pgf@splitbezier@i@ii{\pgf@x\the\pgf@x\pgf@y\the\pgf@y}%
  % P^1_1
  \pgf@xa=.5\pgf@xa\advance\pgf@xa by.5\pgf@xb%
  \pgf@ya=.5\pgf@ya\advance\pgf@ya by.5\pgf@yb%
  % P^1_2
  \pgf@xb=.5\pgf@xb\advance\pgf@xb by.5\pgf@xc%
  \pgf@yb=.5\pgf@yb\advance\pgf@yb by.5\pgf@yc%
  \edef\pgf@splitbezier@ii@iii{\pgf@x\the\pgf@xb\pgf@y\the\pgf@yb}%
  % P^2_0
  \pgf@x=.5\pgf@x\advance\pgf@x by.5\pgf@xa%
  \pgf@y=.5\pgf@y\advance\pgf@y by.5\pgf@ya%
  \edef\pgf@splitbezier@i@iii{\pgf@x\the\pgf@x\pgf@y\the\pgf@y}%
  % P^2_1
  \pgf@xa=.5\pgf@xa\advance\pgf@xa by.5\pgf@xb%
  \pgf@ya=.5\pgf@ya\advance\pgf@ya by.5\pgf@yb%
  \edef\pgf@splitbezier@ii@ii{\pgf@x\the\pgf@xa\pgf@y\the\pgf@ya}%
  % P^3_0
  \pgf@x=.5\pgf@x\advance\pgf@x by.5\pgf@xa%
  \pgf@y=.5\pgf@y\advance\pgf@y by.5\pgf@ya%
  \edef\pgf@splitbezier@i@iv{\pgf@x\the\pgf@x\pgf@y\the\pgf@y}%
  \let\pgf@splitbezier@ii@i\pgf@splitbezier@i@iv
}


% computes the cross product and puts it into \pgfmathresult
\def\pgfmathcrossproduct#1#2{%
  \begingroup
    \pgf@process{#1}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{#2}%
    \pgf@y=\pgf@sys@tonumber\pgf@xa\pgf@y
    \advance\pgf@y by -\pgf@sys@tonumber\pgf@ya\pgf@x
  \pgfmath@returnone\pgf@y
  \endgroup
}

\def\pgfmathdotproduct#1#2{%
  \begingroup
    \pgf@process{#1}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{#2}%
    \pgf@x=\pgf@sys@tonumber\pgf@xa\pgf@x
    \advance\pgf@x by \pgf@sys@tonumber\pgf@ya\pgf@y
  \pgfmath@returnone\pgf@x
  \endgroup
}

\def\pgfmathcrossdot#1#2{%
  \begingroup
    \pgf@process{#1}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{#2}%
    \pgf@xb=\pgf@sys@tonumber\pgf@xa\pgf@x
    \pgf@yb=\pgf@sys@tonumber\pgf@xa\pgf@y
    \advance\pgf@xb by \pgf@sys@tonumber\pgf@ya\pgf@y
    \advance\pgf@yb by -\pgf@sys@tonumber\pgf@ya\pgf@x
    \edef\pgf@temp{%
      \edef\noexpand\pgf@tmp@dot{\pgf@sys@tonumber\pgf@xb}%
      \edef\noexpand\pgf@tmp@cross{\pgf@sys@tonumber\pgf@yb}%
    }%
  \expandafter
  \endgroup\pgf@temp
}

% Calculates abs(\pgf@x) + abs(\pgf@y) in #1
\def\pgfpointtaxicabnorm#1{%
  \ifdim\pgf@x<0pt
    #1=-\pgf@x
  \else
    #1=\pgf@x
  \fi
  \ifdim\pgf@y<0pt
    \advance#1 by -\pgf@y
  \else
    \advance#1 by \pgf@y
  \fi
}

% Computes the normalised tangents of a given Bezier curve and stores them in \pgf@tmp@tang@i and \pgf@tmp@tang@ii.
% Also computes the angles and stores them in  \pgf@tmp@angle@i and \pgf@tmp@angle@ii.
% All degenerate cases are covered. For a triple degenerate curve (all points equal), the vector (1,0) is returned.
\def\pgf@offset@compute@tangents#1#2#3#4{%
  \pgf@process{\pgfpointdiff{#1}{#2}}% unintuitively, this is PTii - PTi
  \pgfpointtaxicabnorm\pgf@xa
  \ifdim\pgf@xa<0.1pt\relax
    % edge case: first point and first control point are equal
    \pgf@process{\pgfpointdiff{#1}{#3}}%
    \pgfpointtaxicabnorm\pgf@xa
    \ifdim\pgf@xa<0.1pt\relax
      % edge case: first three points are equal
      \pgf@process{\pgfpointdiff{#1}{#4}}%
    \fi
  \fi
  \pgfextract@process\pgf@tmp@tang@i{%
    \pgfpointnormalised{}%
    % \pgfpointnormalised stores the angle of the vector in \pgf@tmp
    \global\let\pgf@nfold@tmp\pgf@tmp%
  }%
  \let\pgf@tmp@angle@i\pgf@nfold@tmp%
  \pgf@process{\pgfpointdiff{#3}{#4}}%
  \pgfpointtaxicabnorm\pgf@xa
  \ifdim\pgf@xa<0.1pt\relax
    \pgf@process{\pgfpointdiff{#2}{#4}}%
    \pgfpointtaxicabnorm\pgf@xa
    \ifdim\pgf@xa<0.1pt\relax
      \pgf@process{\pgfpointdiff{#1}{#4}}%
    \fi
  \fi
  \pgfextract@process\pgf@tmp@tang@ii{\pgfpointnormalised{}\global\let\pgf@nfold@tmp\pgf@tmp}%
  \let\pgf@tmp@angle@ii\pgf@nfold@tmp%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Offsetting a simple section %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\pgf@offset@bezier@segment#1#2#3#4#5{%
  % normalise tangents and normals; this avoids overflow issues later, and we need
  % the normal vector to be of length 1 anyway
  \pgf@offset@compute@tangents{#1}{#2}{#3}{#4}%
  \pgf@offset@bezier@segment@{#1}{#2}{#3}{#4}{#5}%
}

% this version assumes that the tangents have been precomputed in \pgf@tmp@tang@i and @ii
\def\pgf@offset@bezier@segment@#1#2#3#4#5{%
  % offset A1
  % compute the normal
  \pgf@tmp@tang@i
  \edef\pgf@tmp@normal@i{\noexpand\pgfqpoint{-\the\pgf@y}{\the\pgf@x}}%
  \pgfextract@process\pgf@bezier@offset@i
    {\pgfpointadd{\pgfpointscale{#5}{\pgf@tmp@normal@i}}{#1}}%
  % offset A4
  \pgf@tmp@tang@ii
  \edef\pgf@tmp@normal@ii{\noexpand\pgfqpoint{-\the\pgf@y}{\the\pgf@x}}%
  \pgfextract@process\pgf@bezier@offset@iv
    {\pgfpointadd{\pgfpointscale{#5}{\pgf@tmp@normal@ii}}{#4}}%
  % now compute A'_2 and A'_3
  \pgf@process{\pgfpointdiff{#1}{#4}}%
  \pgfmathveclen@{\pgf@sys@tonumber\pgf@x}{\pgf@sys@tonumber\pgf@y}%
  \let\pgf@tmp@secantlen\pgfmathresult
  \ifdim\pgf@tmp@secantlen pt<0.1pt\relax
    % Edge case: Either the curve is degenerate to a point or it is not simple.
    % Either way we offset A1 and A4, and preserve the vectors A1A2 and A3A4.
    \pgfutil@packagewarning{tikz-nfold}{first and last point are too close, expect glitches}%
    \pgfextract@process\pgf@bezier@offset@ii
      {\pgfpointadd{\pgf@bezier@offset@i}{\pgfpointdiff{#1}{#2}}}%
    \pgfextract@process\pgf@bezier@offset@iii
      {\pgfpointadd{\pgf@bezier@offset@iv}{\pgfpointdiff{#4}{#3}}}%
  \else
    \pgfextract@process\pgf@tmp@secant{\pgfpointnormalised{}}%
    \pgfmathcrossdot{}{\pgf@tmp@tang@ii}%
     \ifdim\pgf@tmp@dot pt<.5pt\relax%
       % this can only happen in non-simple curves
       \pgfutil@packagewarning{tikz-nfold}{cosine of \pgf@tmp@dot\space clamped to 0.5 in non-simple segment}%
       \def\pgf@tmp@dot{.5}%
    \fi%
    \pgfmathdivide@{\pgf@tmp@cross}{\pgf@tmp@dot}%
    \let\pgf@tmp@tanbeta\pgfmathresult
    \pgfmathcrossdot{\pgf@tmp@secant}{\pgfpointnormalised{\pgfpointdiff{#1}{#2}}}
    % There are cases where we want #5/secantlen to be quite large, so we should not clamp the value here
    % \pgfmathparse{1 + #5/\pgf@tmp@secantlen*(\pgf@tmp@cross - \pgf@tmp@dot*\pgf@tmp@tanbeta)}%
    \pgfmath@offset@calculate@scale{\pgf@tmp@secantlen}{\pgf@tmp@cross}{\pgf@tmp@dot}{\pgf@tmp@tanbeta}{#5}%
    \pgfextract@process\pgf@bezier@offset@ii{%
      \pgfpointadd
        {\pgf@bezier@offset@i}
        {\pgfqpointscale{\pgfmathresult}{\pgfpointdiff{#1}{#2}}}%
    }%
    % third control point
    \pgfmathcrossdot{\pgf@tmp@secant}{\pgf@tmp@tang@i}%
    \ifdim\pgf@tmp@dot pt<.5pt\relax
      \pgfutil@packagewarning{tikz-nfold}{cosine of \pgf@tmp@dot\space clamped to 0.5 in non-simple segment}%
      \def\pgf@tmp@dot{.5}%
    \fi
    \pgfmathdivide@{\pgf@tmp@cross}{\pgf@tmp@dot}%
    \let\pgf@tmp@tanbeta\pgfmathresult
    \pgfmathcrossdot{\pgf@tmp@secant}{\pgfpointnormalised{\pgfpointdiff{#4}{#3}}}%
    % \pgfmathparse{1 + #5/\pgf@tmp@secantlen*(\pgf@tmp@cross - \pgf@tmp@dot*\pgf@tmp@tanbeta)}%
    \pgfmath@offset@calculate@scale{\pgf@tmp@secantlen}{\pgf@tmp@cross}{\pgf@tmp@dot}{\pgf@tmp@tanbeta}{#5}%
    \pgfextract@process\pgf@bezier@offset@iii{%
      \pgfpointadd
        {\pgf@bezier@offset@iv}
        {\pgfqpointscale{\pgfmathresult}{\pgfpointdiff{#4}{#3}}}%
    }%
  \fi
}

% calculates 1+#5/#1*(#2-#3*#4)
% #1 = secantlen
% #2 = cross
% #3 = dot
% #4 = tanbeta
% #5 = #5 (offset)
\def\pgfmath@offset@calculate@scale#1#2#3#4#5{%
  \begingroup
    \pgfmathmultiply@{#3}{#4}%
    \pgfmathsubtract@{#2}{\pgfmathresult}%
    \let\pgfmath@temp\pgfmathresult
    \pgfmathreciprocal@{#1}%
    \pgfmathmultiply@{\pgfmathresult}{\pgfmath@temp}%
    \pgfmathmultiply{\pgfmathresult}{#5}%
    \pgfmathadd@{\pgfmathresult}{1}%
    \pgfmath@smuggleone\pgfmathresult
  \endgroup
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Subdividing and offsetting %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Maximum level of recursion. The theoretical limit to the number of subdivisions in the final curve
% is given by 2^\pgf@offset@max@recursion
\newcount\pgf@offset@max@recursion
\pgf@offset@max@recursion=4

%
% Subdivides a Bezier curve into "simple" segments (according to the definition below),
% offsets the segments, and draws them.  Because offsetting also involves relocating
% the starting points, these macros come in two variants: with and without a \pgfpathmoveto{}
% to the new starting point.
%
% Interface:
% #1-#4: control points of the whole Bezier curve
% #5: offset

\def\pgfoffsetcurve#1#2#3#4#5{%
  \pgfoffsetcurvecallback{#1}{#2}{#3}{#4}{#5}{\pgf@nfold@callback@move}%
}
\def\pgfoffsetcurvenomove#1#2#3#4#5{%
  \pgfoffsetcurvecallback{#1}{#2}{#3}{#4}{#5}{\pgf@nfold@callback@nomove}%  
}

% Arguments:
% #1-#4: control points of the segment
% #5: =0 if this is the first segment of the curve, =1 otherwise
%   (checking for #5=0 allows us to draw the curve without interruptions)
\def\pgf@nfold@callback@move#1#2#3#4#5{%
  \if#50\pgfpathmoveto{#1}\fi%
  \pgfpathcurveto{#2}{#3}{#4}%
}
% this version never does a moveto at the start. Useful for drawing a path consisting of
% multiple Bezier curves.
\def\pgf@nfold@callback@nomove#1#2#3#4#5{\pgfpathcurveto{#2}{#3}{#4}}

% This macro subdivides and offsets a curve and executes a given callback on every offset simple segment.
% #1-#4: control points of the segment
% #5: =0 if this is the first segment of the curve, =1 otherwise
% #6: callback (see \pgf@nfold@callback@move) for the parameters
\def\pgfoffsetcurvecallback#1#2#3#4#5#6{%
  \edef\pgf@offset@tmp@callback##1##2##3##4##5{%
    \noexpand\pgf@offset@bezier@segment{##1}{##2}{##3}{##4}{#5}%
    \noexpand#6{\noexpand\pgf@bezier@offset@i}{\noexpand\pgf@bezier@offset@ii}{\noexpand\pgf@bezier@offset@iii}{\noexpand\pgf@bezier@offset@iv}{##5}%
  }
  \pgf@subdividecurve{#1}{#2}{#3}{#4}{\pgf@offset@max@recursion}{0}{\pgf@offset@tmp@callback}%
}


% This macro subdivides (but does not offset) a curve and executes a callback on every simple segment.
% #1-#4: control points
% #5: recursion limit (decreases on every recursive call)
% #6: =0 if this is the start of the curve, =1 otherwise
% #7: callback for output (see above)
\newif\ifpgf@offset@subdivide
\def\pgf@subdividecurve#1#2#3#4#5#6#7{%
  \begingroup%
    \pgfextract@process\pgf@ctrl@i{#1}%
    \pgfextract@process\pgf@ctrl@ii{#2}%
    \pgfextract@process\pgf@ctrl@iii{#3}%
    \pgfextract@process\pgf@ctrl@iv{#4}%
    \pgf@offset@compute@tangents{\pgf@ctrl@i}{\pgf@ctrl@ii}{\pgf@ctrl@iii}{\pgf@ctrl@iv}%
    \pgf@subdividecurve@{#5}{#6}{#7}%
  \endgroup%
}

% This macro assumes that the curve is defined in \pgf@ctrl@i-\pgf@ctrl@iv
% and that its tangents have already been computed.
\def\pgf@subdividecurve@#1#2#3{%
  \pgf@offset@subdividefalse%
  \c@pgf@counta=#1\relax
  \advance\c@pgf@counta by -1
  % Use the non-degenerate tangents for the simplicity check
  \pgfextract@process\pgf@itoiv{\pgfpointdiff{\pgf@ctrl@i}{\pgf@ctrl@iv}}%
  \pgfmathcrossproduct{\pgf@itoiv}{\pgf@tmp@tang@i}%
  \let\firstcross\pgfmathresult
  \pgfmathcrossproduct{\pgf@itoiv}{\pgf@tmp@tang@ii}%
  % First simplicity check: Are A2 and A3 on the same side of the A1-A4 line?
  % -> compute the sign of the cross products, use the sign function to avoid overflows
  % just give it a pass if one of them is zero, hence 2 and 3 at the end
  \ifnum
    \ifdim   \firstcross pt<0pt -1\else\ifdim   \firstcross pt>0pt 1\else 2\fi\fi
   =\ifdim\pgfmathresult pt<0pt -1\else\ifdim\pgfmathresult pt>0pt 1\else 3\fi\fi
  \relax % the \relax is important!
    \pgf@offset@subdividetrue%
  \else%
    % Second simplicity check: How large is the angle between the tangents in A1 and A4?
    \pgfmathdotproduct{\pgf@tmp@tang@i}{\pgf@tmp@tang@ii}%
    \ifdim\pgfmathresult pt<.5pt\relax%
      \pgf@offset@subdividetrue%
    \else
      % Third simplicity check: Put a limit on the lengths of the i-ii and iii-iv vectors combined
      \pgf@itoiv
      \pgfmathveclen@{\pgf@sys@tonumber\pgf@x}{\pgf@sys@tonumber\pgf@y}%
      \pgf@xa=\pgfmathresult pt
      \pgf@process{\pgfpointdiff{\pgf@ctrl@i}{\pgf@ctrl@ii}}%
      \pgfmathveclen@{\pgf@sys@tonumber\pgf@x}{\pgf@sys@tonumber\pgf@y}%
      \pgf@xb=\pgfmathresult pt
      \pgf@process{\pgfpointdiff{\pgf@ctrl@iii}{\pgf@ctrl@iv}}%
      \pgfmathveclen@{\pgf@sys@tonumber\pgf@x}{\pgf@sys@tonumber\pgf@y}%
      \advance\pgf@xb by \pgfmathresult pt
      % veclen(iv-i) < veclen(ii-i) + veclen(iv-iii)
      \ifdim\pgf@xa<\pgf@xb
        \pgf@offset@subdividetrue
      \fi
    \fi%
  \fi%
  \ifpgf@offset@subdivide%
    \ifnum\c@pgf@counta<0%
      % We hit the recursion limit but the segment is not simple
      \pgfutil@packagewarning{tikz-nfold}{Recursion limit reached, glitches may occur. %
        Consider increasing \string\pgf@offset@max@recursion}%
      % Try to offset the curve anyway. The result will not be precise,
      % but the code is sufficiently robust to not crash
      #3{\pgf@ctrl@i}{\pgf@ctrl@ii}{\pgf@ctrl@iii}{\pgf@ctrl@iv}{#2}%
    \else
      % split the non-simple segment and execute recursive calls
      \pgf@halfsplitbezier{\pgf@ctrl@i}{\pgf@ctrl@ii}{\pgf@ctrl@iii}{\pgf@ctrl@iv}%
      % compute the tangent at the spitting point; this vector is only zero if the curve
      % is degenerate to a point, in which case we can't compute the tangent anyway
      \pgfextract@process\pgf@middletangent{%
        \pgfpointnormalised{\pgfpointdiff{\pgf@splitbezier@i@iii}{\pgf@splitbezier@i@iv}}}%
      \begingroup%
        % we need a group to avoid overwriting variables in recursive calls
        \let\pgf@tmp@tang@ii\pgf@middletangent%
        \let\pgf@ctrl@i\pgf@splitbezier@i@i%
        \let\pgf@ctrl@ii\pgf@splitbezier@i@ii%
        \let\pgf@ctrl@iii\pgf@splitbezier@i@iii%
        \let\pgf@ctrl@iv\pgf@splitbezier@i@iv%
        % pass on the "start of the curve flag" only to the first term
        \pgf@subdividecurve@{\c@pgf@counta}{#2}{#3}%
      \endgroup%
      \begingroup%
        \let\pgf@tmp@tang@i\pgf@middletangent%
        \let\pgf@ctrl@i\pgf@splitbezier@ii@i%
        \let\pgf@ctrl@ii\pgf@splitbezier@ii@ii%
        \let\pgf@ctrl@iii\pgf@splitbezier@ii@iii%
        \let\pgf@ctrl@iv\pgf@splitbezier@ii@iv%
        \pgf@subdividecurve@{\c@pgf@counta}{1}{#3}%
      \endgroup%
    \fi%
  \else%
    % curve is simple
    #3{\pgf@ctrl@i}{\pgf@ctrl@ii}{\pgf@ctrl@iii}{\pgf@ctrl@iv}{#2}%
  \fi%
}


%
% Offsetting straight lines
% -------------------------
%
% For convenience we also provide macros that offset straight lines. These also come in two variants
% similar to the macros for curves.
%
\def\pgfoffsetline#1#2#3{%
  \pgfmathparse{#3}%
  \pgfoffsetline@{#1}{#2}{\pgfmathresult}{\pgfpointnormalised{\pgfpointdiff{#1}{#2}}}%
}

% a quicker version in case we already know the tangent and #3 is a number without unit
\def\pgfoffsetline@#1#2#3#4{%
  \pgfqpointscale{#3}{#4}%
  \pgf@xc=-\pgf@y
  \pgf@yc=\pgf@x
  \pgfpathmoveto{\pgfpointadd{#1}{\pgfqpoint{\pgf@xc}{\pgf@yc}}}%
  \pgfpathlineto{\pgfpointadd{#2}{\pgfqpoint{\pgf@xc}{\pgf@yc}}}%
}

\def\pgfoffsetlinenomove#1#2#3{%
  \pgfoffsetlinenomove@{#1}{#2}{#3}{\pgfpointnormalised{\pgfpointdiff{#1}{#2}}}%
}

\def\pgfoffsetlinenomove@#1#2#3#4{%
  \pgfqpointscale{#3}{#4}%
  \pgf@xc=-\pgf@y
  \pgf@yc=\pgf@x
  \pgfpathlineto{\pgfpointadd{#2}{\pgfqpoint{\pgf@xc}{\pgf@yc}}}%
}


==> pgflibrarynfold.code.tex <==
%% pgflibrarynfold.code.tex
%% Copyright 2023 Jonathan Schulz
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3c
% of this license or (at your option) any later version.
% The latest version of this license is in
% http://www.latex-project.org/lppl.txt
% and version 1.3c or later is part of all distributions of LaTeX
% version 2008-05-04 or later.
%
% This work has the LPPL maintenance status 'maintained'.
%
% The Current Maintainer of this work is Jonathan Schulz.
%
% This work consists of the files pgflibrarybezieroffset.code.tex,
% tikzlibrarynfold.code.tex, tikz-nfold-doc.tex, and tikz-nfold-doc.pdf.


\usepgflibrary{offsetpath}

%
% Iterating over the parsed and processed soft path
% -------------------------------------------------
%

\newcount\pgf@nfold@index
\def\pgf@nfold@run@loop{%
  \pgf@nfold@index=\pgf@nfold@order%
  \pgf@nfold@run@loop@%
}

\def\pgf@nfold@run@loop@{%
  \pgf@nfold@loop@inner%
  \advance\pgf@nfold@index by -1\relax
  \ifnum\pgf@nfold@index>0\relax%
    \pgf@nfold@run@loop@%
  \fi%
}

\def\pgf@nfold@loop@inner{%
  \pgfmathsetmacro{\pgf@nfold@shift@fraction}%
    {-1+2*(\pgf@nfold@index-1)/(\pgf@nfold@order-1)}%
  % Do not store shiftamount as a length (i.e. with pt) because we want to use it in \pgfqpointscale{}{}
  \pgfmathsetmacro{\pgf@nfold@shiftamount}{\pgf@nfold@hwidth*\pgf@nfold@shift@fraction}
  % Transformations are already baked into the path; without this call, they would be applied twice
  \pgftransformreset%
  \parsedpath%
  \pgfsyssoftpath@flushcurrentpath%
  \pgf@up@action%
}

% Computes both the width of the component lines into \pgf@x and the distance
% from the center to the outermost line centers into \pgf@y
% from the current values of \pgflinewidth and \pgfinnerlinewidth.
\def\pgf@nfold@compute@widths@from@double{
    \pgf@x=\pgflinewidth\relax%
    \pgf@y=\pgf@x\relax%
    \advance\pgf@x-\pgfinnerlinewidth\relax%
    \advance\pgf@y+\pgfinnerlinewidth\relax%
    \pgf@x=.5\pgf@x\relax%
    \pgf@y=.25\pgf@y\relax%
}

\def\pgf@nfold@render@cached@softpath{%
  \pgfscope% must use a scope, otherwise we break the arrow tips
    % Compute the full and constituent part line widths
    \pgf@nfold@compute@widths@from@double%
    \pgfsetlinewidth\pgf@x%
    \edef\pgf@nfold@hwidth{\the\pgf@y}%
    \pgfprocessround{\pgf@nfold@cachedpath}{\pgf@nfold@cachedpath}% remove tokens from the soft path
    \pgf@nfold@parsearrows%
    \pgf@nfold@parsesoftpath{\pgf@nfold@cachedpath}{\parsedpath}%
    \pgf@nfold@run@loop%
  \endpgfscope%
}

%
% pgf keys
% --------
%

\pgfkeys{
  /pgf/nfold/.code={%
    \pgf@nfold@order=#1\relax%
    \ifnum\pgf@nfold@order<1\relax%
      \pgfutil@packageerror{tikz-nfold}{The key /pgf/nfold must take a value of at least 1, got \the\pgf@nfold@order}{}%
    \fi%
    % If nfold > numcached AND intersections is not loaded AND we draw an Implies tip, we get an error.
    % We check the first two conditions now and set the respective flag
    \ifnum\pgf@nfold@order>\pgf@nfold@intersec@numcached\relax
      \ifdefined\pgfintersectionofpaths\else
        \pgf@nfold@intersectionsnotloadedtrue
      \fi
    \fi
  },
  /pgf/nfold/.default=2
}

\endinput

==> pgflibraryoffsetpath.code.tex <==
%% pgflibraryoffsetpath.code.tex
%% Copyright 2023 Jonathan Schulz
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3c
% of this license or (at your option) any later version.
% The latest version of this license is in
% http://www.latex-project.org/lppl.txt
% and version 1.3c or later is part of all distributions of LaTeX
% version 2008-05-04 or later.
%
% This work has the LPPL maintenance status 'maintained'.
%
% The Current Maintainer of this work is Jonathan Schulz.
%
% This work consists of the files pgflibrarybezieroffset.code.tex,
% tikzlibrarynfold.code.tex, tikz-nfold-doc.tex, and tikz-nfold-doc.pdf.

\usepgflibrary{bezieroffset}


%
% General idea
% ============
%
% In order to offset a path, we must first analyse and slightly modify it. For example,
% the start and end points of segments need to be relocated slightly in order to make room
% for the joins, and most curves must be subdivided for the offsetting algorithm. To avoid
% redundant computations in n-fold paths, we pre-compute as much data as possible and store
% all this information in a "parsed path" macro. The structure of the parsed path resembles
% the structure of a pgf softpath, but it consists of different tokens.
%
% Parsing is a two-step process: We iterate over the path in the first step and separate
% it into connected sub-paths. This is necessary for closed paths, because we need to know
% the location of the \pgfpathclose-segment in order to correctly offset the first segment
% of this connected sub-path.
%
% Once we have parsed a connected sub-path and stored all the information necessary, the
% second step, called _processing_, begins. This involves relocating start and end points
% to make room for joins, storing all the information for a given join, subdividing curves,
% and handling a number of edge cases.
%
% The resulting parsed and processed path (shortened to "parsed path") consists of tokens
% like \pgf@nfold@token@lineto. Once a few macros are defined that control by how much
% the curve should be offset, the parsed path can be invoked directly.
%



%
% Intercepting join settings
% --------------------------
%
% The current settings of the line joins are not stored in any TeX registers; instead, direct system
% calls are made to apply the settings. Therefore, we need to modify the pgf macros in order
% to cache the current settings.
%

% The initial value is miter limit=10 according to the pdf standard (it is not set by pgf)
\gdef\pgf@nfold@cached@miterlimit{10}
\let\pgf@nfold@old@miterlimit\pgfsetmiterlimit
\def\pgfsetmiterlimit#1{%
  \pgf@nfold@old@miterlimit{#1}%
  \edef\pgf@nfold@cached@miterlimit{#1}%
}

% default line join is "miter"
\global\let\pgf@cached@linejoin=m% % b = bevel, m=miter, r=round
\let\pgf@nfold@old@setbeveljoin\pgfsetbeveljoin
\let\pgf@nfold@old@setmiterjoin\pgfsetmiterjoin
\let\pgf@nfold@old@setroundjoin\pgfsetroundjoin
\def\pgfsetbeveljoin{%
  \pgf@nfold@old@setbeveljoin%
  % do NOT change this globally! Needs to be changed back at the end of groups for scoping reasons
  \let\pgf@cached@linejoin=b%
}
\def\pgfsetmiterjoin{%
  \pgf@nfold@old@setmiterjoin%
  \let\pgf@cached@linejoin=m%
}
\def\pgfsetroundjoin{%
  \pgf@nfold@old@setroundjoin%
  \let\pgf@cached@linejoin=r%
}


%
% Joining offset lines
% --------------------
%
% One of the more difficult aspects is joining the segments of an offset path. Without this step,
% the path would be interrupted or self-intersect whenever there is a non-zero angle between
% two segments. This code reproduces the existing line joins "bevel", "miter" and "round".
%

\def\pgf@nfold@miterjoin{
  % The tip of the miter join is computed starting from the original (unshifted) centre of the join;
  % we then move orthorgonal to the average of the old and new angle
  \pgfpathlineto{
    \pgfpointadd{\pgf@nfold@join@centre}{%
      \pgfpointpolar{\pgf@nfold@firstang+.5*\pgf@nfold@deltaphi+90}% do not change
        {\pgf@nfold@shiftamount/cos(.5*\pgf@nfold@deltaphi)}%
    }%
  }%
}

\def\pgf@nfold@beveljoin{
  % The bevel join for one component line consists of three parts:
  % 1) an extension of the ingoing line,
  % 2) a middle line, angled at the average of the incoming and outgoing line,
  % 3) an extension of the outgoing line.
  % Different components of the ingoing and outgoing lines have a constant distance from each other.
  % For a good-looking output, the mittle parts of the component lines thus should also have a constant distance,
  % which is a non-trivial condition. To generate such an output the outer lines get a bevel-like join
  % and the inner lines get a miter-like join; the threshold depends on deltaphi.
  % We first compute by how much the outermost line must be continued from the beginning of the join.
  % The protrusion amount must be lowered by a little bit for a rather complicated reason: The offset would be
  % dead on if the outermost offset line were centered on the _edge_ of the wide line, but we want to draw 
  % the outside line _fully inside_ the wide line. The factor of tan(deltaphi/4) can be derived, but is not obvious.
  \pgfmathsetlengthmacro{\bevelouterprotrusion}%
    {\pgf@nfold@shortenstartjoin pt - .5*\pgflinewidth*abs(tan(.25*\pgf@nfold@deltaphi))}
  % The following applies to middle lines only: We compute by how much they need to be shortened so the distance
  % between the lines in the join is correct.
  \pgfmathsetmacro{\bevelshorten}{2*\insidepercentage*abs(tan(.25*\pgf@nfold@deltaphi))}
  % This threshold decides if the inside line has a bevel or a miter join
  \pgfmathparse{\bevelshorten < abs(sin(.5*\pgf@nfold@deltaphi))}
  \ifnum\pgfmathresult=1\relax
    \pgfmathsetlengthmacro{\bevelextension}{\bevelouterprotrusion-\bevelshorten*\pgf@nfold@hwidth}
    \pgfpointadd{\pgf@nfold@join@start}{\pgfpointpolar{\pgf@nfold@firstang}{\bevelextension}}
    \pgfpathlineto{}
    \pgfpointadd{\pgf@nfold@join@end}{\pgfpointpolar{\pgf@nfold@secondang}{-\bevelextension}}
    \pgfpathlineto{}
  \else
    \pgf@nfold@miterjoin
  \fi
}

\def\pgf@nfold@roundjoin{
  % The outer half of the lines get arcs, the others get miters
  \ifdim\insidepercentage pt<.5pt\relax
    \pgfpointadd{\pgf@nfold@join@start}{\pgfpointpolar{\pgf@nfold@firstang}{\pgf@nfold@shortenstartjoin}}
    \pgfpathlineto{}
    % TODO needs unit tests for all cases left, right, across the 360 gap etc.
    \pgfmathsetmacro\pgf@tmp@firstang{\pgf@nfold@firstang+90*\turnindicator}
    \pgfpatharc%
      {\pgf@tmp@firstang}%
      {\pgf@tmp@firstang+\pgf@nfold@deltaphi}%
      {abs(\pgf@nfold@shift@fraction)*\pgf@nfold@hwidth}%
  \else
    \pgf@nfold@miterjoin
  \fi
}

% The handler that will be added to the parsed path
% #1: The centre of the join
% #2: The end point of the first segment
% #3: The starting point of the second segment
% #4: The angle of the first segment
% #5: The angle of the second segment
% #6: deltaphi in the range [-180, 180]
% #7: the distance between #1 and #2
% #8: the join + finish macro
\def\pgf@nfold@token@join#1#2#3#4#5#6#7#8{%
  \def\pgf@nfold@join@centre{#1}%
  \def\pgf@nfold@join@prevend{#2}%
  \def\pgf@nfold@join@nextstart{#3}%
  \def\pgf@nfold@firstang{#4}%
  \def\pgf@nfold@secondang{#5}%
  % Offset the start and end of this join
  \pgfextract@process\pgf@nfold@join@start{%
    \pgfpointadd{#2}{\pgfpointpolar{\pgf@nfold@firstang+90}{\pgf@nfold@shiftamount}}}%
  \pgfextract@process\pgf@nfold@join@end{%
    \pgfpointadd{#3}{\pgfpointpolar{\pgf@nfold@secondang+90}{\pgf@nfold@shiftamount}}}%
  \pgf@process{\pgfpointdiff{\pgf@nfold@join@start}{\pgf@nfold@join@end}}
  % Check if the start of this segment is very close to the end of the previous segment.
  % In that case we don't need a join at all
  \pgfpointtaxicabnorm\pgfutil@tempdima
  \ifdim\pgfutil@tempdima>0.1pt\relax
    \def\pgf@nfold@deltaphi{#6}%
    \def\pgf@nfold@shortenstartjoin{#7}%
    % First step: Check if left or right turn (-1=left, 1=right)
    \ifdim\pgf@nfold@deltaphi pt<0pt
      \def\turnindicator{1}
    \else
      \def\turnindicator{-1}
    \fi
    % \insidepercentage: between 0.0 and 1.0;
    % 0=no distance to cover in the join, 1=maximum distance to cover
    \pgfutil@tempdima=\pgf@nfold@shift@fraction pt\relax
    \pgfutil@tempdima=\turnindicator\pgfutil@tempdima
    \advance\pgfutil@tempdima by-1pt\relax
    \pgfutil@tempdima=-.5\pgfutil@tempdima
    % \insidepercentage  = .5 * (1 - \turnindicator*\pgf@nfold@shift@fraction)
    \edef\insidepercentage{\pgf@sys@tonumber\pgfutil@tempdima}%
    #8%
  \fi
}


%
% Join handler
%
\def\pgf@nfold@process@join{%
  % \pgf@xa := abs(deltaphi@start)
  \pgf@xa=\pgf@nfold@deltaphi@start pt\relax
  \ifdim\pgf@xa<0pt\relax
    \pgf@xa=-\pgf@xa
  \fi
  % Skip the entire join if abs(deltaphi) is too small
  \ifdim\pgf@xa>1pt\relax
    \edef\pgf@nfold@jointype{\pgf@cached@linejoin}
    \if\pgf@cached@linejoin m% \ifx is not needed because both are only one character
      % miter join
      % First we implement the miter limit: If the angle is too sharp, the miter join is replaced
      % by a bevel join. This is controlled e.g. by /tikz/miter limit=..., initially 10.
      \pgf@xa=.5\pgf@xa
      \pgfmathcos@{\pgf@sys@tonumber\pgf@xa}
      \pgf@xa=\pgfmathresult pt\relax
      \pgf@xa=\pgf@nfold@cached@miterlimit\pgf@xa
      % Switch to bevel if miterlimit*cos(.5*abs(deltaphi)) <= 1
      \ifdim\pgf@xa>1pt\relax
        \def\pgf@nfold@tmp@joinmacro{\pgf@nfold@miterjoin}
      \else
        \def\pgf@nfold@tmp@joinmacro{\pgf@nfold@beveljoin}
      \fi
    \else
      \if b\pgf@cached@linejoin\relax
        \def\pgf@nfold@tmp@joinmacro{\pgf@nfold@beveljoin}
      \else
        \def\pgf@nfold@tmp@joinmacro{\pgf@nfold@roundjoin}
      \fi
    \fi
    % The last parameter is a macro to be called when this segment of the join is non-trivial.
    % It consists of
    %   - the macro to actually draw the join,
    %   - either finish@normal or finish@edgecase.
    \edef\pgf@nfold@macrotoadd{%
      \noexpand\pgf@nfold@token@join{\pgf@nfold@cur@first}{\pgf@nfold@prev@segment@end}
        {\pgf@nfold@cur@movedfirst}{\pgf@nfold@prev@angle@ii}{\pgf@nfold@cur@angle@i}%
        {\pgf@nfold@deltaphi@start}{\pgf@nfold@shortenstartjoin}{%
          \expandafter\noexpand\pgf@nfold@tmp@joinmacro%
          \expandafter\noexpand\ifpgf@nfold@closejoinsedgecase%
            \pgf@nfold@token@finish@edgecase{\pgf@nfold@cur@movedlast}%
          \else%
            \pgf@nfold@token@finish@normal%
          \fi%
        }%
    }%
    \pgf@nfold@addmacro\pgf@parsed@cur@conn@seg%
  \fi% end if abs(deltaphi) > 1
}


% All non-trivial joins connect to the end of the join, which is the starting point of the next segment.
% Note that this entire macro is skipped by if the start and end of the join coincide, so we never create a zero length segment here.
%
% There is one edge case here: If two subsequent joins are so close that \pgf@nfold@cur@movedlast
% and \pgf@nfold@cur@movedfirst exchange places *and* we are on the outside of the first join 
% (implying that we are on the inside of the second join), the first join must not connect all the way to
% to \pgf@nfold@cur@movedfirst, because that would overshoot the second join. Instead we connect to
% \pgf@nfold@cur@movedlast (which is *closer* to the first join than \pgf@nfold@cur@movedfirst in this edge case).
% To accomodate for the vertical offset we connect to \pgf@nfold@join@end which is the vertical
% offset of \pgf@nfold@cur@movedlast by definition.
\def\pgf@nfold@token@finish@normal{%
  \pgfpathlineto{\pgf@nfold@join@end}%
}

% parameter #1: @movedlast of the next segment
\def\pgf@nfold@token@finish@edgecase#1{%
  \pgf@nfold@join@end%
  \ifdim\insidepercentage pt<.5pt\relax%
    \pgf@process{\pgfpointadd{#1}{\pgfpointpolar{\pgf@nfold@secondang+90}{\pgf@nfold@shiftamount}}}
  \fi%
  \pgfpathlineto{}%
}


%
% Main rendering pipeline
% -----------------------
%

% This stores whether the current segment should begin with a moveto to its offset
\newif\ifpgf@nfold@continuesegment
% This stores whether we are in some edge case of very close joins, see below for details
\newif\ifpgf@nfold@closejoinsedgecase
% This stores whether we are in an error case where we need to avoid dividing by zero
\newif\ifpgf@nfold@angletoosharp
% This stores whether we need the intersections library for an arrow tip but it is not loaded
\newif\ifpgf@nfold@intersectionsnotloaded
% This stores whether the currently processed connected sub-path is the final one on this path
\newif\ifpgf@nfold@lastconnsubpath


\def\pgf@nfold@process@segment{%
  \if\pgf@nfold@cur@visible0
    % first, last and moveto are invisible
    \if\pgf@nfold@cur@type m
      % We don't need to do anything for a moveto; if a visible segment follows, it will move to
      % its starting location by itself. However, we might need to draw the arrow tip extension
      % at the start (if present).
      % Draw a tip extension only if all of the following conditions are met:
      % 1. There is an Implies tip at the start of this path
      % 2. We are currently on the last connected sub-path of this path
      % 3. The next segment is visible
      % 4. This moveto is the first segment on this path
      \if\pgf@nfold@start@arrowcode1
        \ifpgf@nfold@lastconnsubpath
          \if\pgf@nfold@prev@type f
            \if\pgf@nfold@next@visible1
              \edef\pgf@nfold@macrotoadd{%
                \noexpand\pgf@nfold@extendtotip{s}{\pgf@nfold@cur@last}{\pgf@nfold@next@angle@i}
              }%
              \pgf@nfold@addmacro\pgf@parsed@cur@conn@seg%
              % hack: We make the next segment believe that this segment was a lineto
              % so the path does not get interrupted
              \let\pgf@nfold@cur@type l
              \let\pgf@nfold@cur@visible1
              \let\pgf@nfold@cur@angle@ii\pgf@nfold@next@angle@i
              \let\pgf@nfold@cur@tang@ii\pgf@nfold@next@tang@i
              \def\pgf@nfold@deltaphi@end{0}
              \pgf@nfold@angletoosharpfalse
            \fi
          \fi%
        \fi
      \fi
    \fi%
  \else%
    \let\pgf@nfold@cur@movedfirst\pgf@nfold@cur@first
    \let\pgf@nfold@cur@movedlast\pgf@nfold@cur@last
    %%% Step 1: Make room for joins if necessary
    % In order to make room for the join, it may be necessary to shorten the current segment
    % at the start and/or the end. In here we store by how much the segment needs to be shortened.
    \def\pgf@nfold@shortenstartjoin{0}
    \def\pgf@nfold@shortenendjoin{0}
    \pgf@nfold@closejoinsedgecasefalse
    % Step 1.1: Make room for the join at the start if needed
    \if\pgf@nfold@prev@visible0
      \pgf@nfold@continuesegmentfalse
    \else
      \pgf@nfold@continuesegmenttrue
      % deltaphi@start can be recycled from deltaphi@end;
      % \ifpgf@nfold@angletoosharp is also still set
      \let\pgf@nfold@deltaphi@start\pgf@nfold@deltaphi@end
      % set \pgf@xb := abs(deltaphi@start)
      \pgf@xb=\pgf@nfold@deltaphi@start pt\relax
      \ifdim\pgf@xb<0pt\relax
        \pgf@xb=-\pgf@xb
      \fi
      \ifpgf@nfold@angletoosharp\else
        \ifdim\pgf@xb>0.5pt\relax
          % make room for the start join if the angle is nonzero;
          % shortenstartjoin := hwidth*tan(.5*abs(deltaphi@start))
          \pgf@yb=.5\pgf@xb
          \pgfmathtan@{\pgf@sys@tonumber\pgf@yb}
          \pgf@yb=\pgf@nfold@hwidth\relax
          \pgf@yb=\pgfmathresult\pgf@yb
          \edef\pgf@nfold@shortenstartjoin{\pgf@sys@tonumber\pgf@yb}
          \pgfextract@process\pgf@nfold@cur@movedfirst{%
            \pgfpointadd{\pgf@nfold@cur@first}%
                        {\pgfqpointscale{\pgf@nfold@shortenstartjoin}{\pgf@nfold@cur@tang@i}}}%
          % If the current segment is a curve, we need to relocate @supporta point as well,
          % as otherwise the @first point could overtake it
          \if\pgf@nfold@cur@type c
            \pgf@process{\pgfpointdiff{\pgf@nfold@cur@first}{\pgf@nfold@cur@supporta}}
            \pgfmathveclen@{\pgf@sys@tonumber\pgf@x}{\pgf@sys@tonumber\pgf@y}
            \ifdim\pgfmathresult pt>0.1pt\relax
              % regular curves (supporta != first):
              % Increase dist(first, supporta) to sqrt(a^2 + b^2) where a=dist(first, supporta) and b=shortenstart. This way, the order of first and supporta is guaranteed to be preserved, and the change to supporta is as small as reasonably possible.
              \pgfmathveclen@{\pgfmathresult}{\pgf@sys@tonumber\pgf@yb}
              \pgfextract@process\pgf@nfold@cur@supporta{\pgfpointadd%
                {\pgf@nfold@cur@first}%
                {\pgfqpointscale{\pgfmathresult}{\pgf@nfold@cur@tang@i}}}%
            \else
              % special treatment for singular curves (supporta = first) to avoid rounding error glitches.
              % In this special case, a slight corner at the end of the join is unavoidable unless we
              % also relocate @supportb, which may have unintended side effects
              \let\pgf@nfold@cur@supporta\pgf@nfold@cur@movedfirst
            \fi
          \fi
        \fi
      \fi
    \fi
    % Step 1.2: Make room for the join at the end if needed
    \if\pgf@nfold@next@visible1
      % Compute the angle difference at the end (between -180 and +180 degrees)
      % using \pgfmathsubtract@ is more readable and no less efficient than computing this manually
      \pgfmathsubtract@{\pgf@nfold@next@angle@i}{\pgf@nfold@cur@angle@ii}
      \pgf@nfold@clampangle
      \edef\pgf@nfold@deltaphi@end{\pgfmathresult}
      \pgf@xb=\pgf@nfold@deltaphi@end pt\relax
      \ifdim\pgf@xb<0pt\relax
        \pgf@xb=-\pgf@xb
      \fi
      \ifdim\pgf@xb>178pt\relax
        \pgfutil@packagewarning{tikz-nfold}{Angle too sharp, expect visual errors}
        \pgf@nfold@angletoosharptrue
      \else
        \pgf@nfold@angletoosharpfalse
        \ifdim\pgf@xb>0.5pt\relax
           % make room for the start join if the angle is nonzero
          % shortenendjoin := hwidth*tan(.5*abs(deltaphi@end))
          \pgf@yb=.5\pgf@xb
          \pgfmathtan@{\pgf@sys@tonumber\pgf@yb}
          \pgf@yb=\pgf@nfold@hwidth\relax
          \pgf@yb=\pgfmathresult\pgf@yb
          \edef\pgf@nfold@shortenendjoin{\pgf@sys@tonumber\pgf@yb}
          \pgf@yb=-\pgf@yb
          \pgfextract@process\pgf@nfold@cur@movedlast{%
            % the use of the minus sign is fine here because \pgf@nfold@shortenendjoin >= 0.0
            \pgfpointadd{\pgf@nfold@cur@last}%
              {\pgfqpointscale{-\pgf@nfold@shortenendjoin}{\pgf@nfold@cur@tang@ii}}}%
          \pgfextract@process\pgf@nfold@cur@movedlast{%
            \pgfpointadd{\pgf@nfold@cur@last}%
              {\pgfqpointpolar{\pgf@nfold@cur@angle@ii}{\pgf@yb}}}%
          \if\pgf@nfold@cur@type c
            % Same procedure as above: relocate supportb if we have a curve
            \pgf@process{\pgfpointdiff{\pgf@nfold@cur@supportb}{\pgf@nfold@cur@last}}
            \pgfmathveclen@{\pgf@sys@tonumber\pgf@x}{\pgf@sys@tonumber\pgf@y}
            \ifdim\pgfmathresult pt>0.1pt\relax
              \pgfmathveclen@{\pgfmathresult}{\pgf@sys@tonumber\pgf@yb}
              \pgfextract@process\pgf@nfold@cur@supportb{\pgfpointadd%
                {\pgf@nfold@cur@last}%
                % can use qpointscale and a minus because \pgfmathresult is guaranteed to be positive
                {\pgfqpointscale{-\pgfmathresult}{\pgf@nfold@cur@tang@ii}}}%
            \else
              \let\pgf@nfold@cur@supportb\pgf@nfold@cur@movedlast
            \fi
          \fi
        \fi
      \fi
      % Step 1.3: Detect an edge case
      % This edge case appears whenever the current segment is such a short line that we would
      % have to reduce its length to less than zero to make room for the joins. In such cases,
      % the line is not drawn at all, and slight modifications must be made to the joins to ensure
      % a correct output (i.e. one join is immediately followed by the next without a segment in between).
      %
      % This edge case can appear for curves as well, but they are much harder to deal with.
      \if\pgf@nfold@cur@type l
        % No need to check for \pgf@nfold@inputsegmentclosepath as it should not be followed by any further segments
        % Now: Check if the total amount of shortening is larger than the length of the segment
        \pgf@process{\pgfpointdiff{\pgf@nfold@cur@first}{\pgf@nfold@cur@last}}
        \pgfmathveclen@{\pgf@sys@tonumber\pgf@x}{\pgf@sys@tonumber\pgf@y}
        \pgf@xa=\pgf@nfold@shortenstartjoin pt\relax
        \advance\pgf@xa by\pgf@nfold@shortenendjoin pt\relax
        \ifdim\pgf@xa>\pgfmathresult pt\relax
          \pgf@nfold@closejoinsedgecasetrue
        \fi
      \fi
    \fi% end if next segment visible
    %
    % Step 2.1: Draw the join at the start if applicable
    %
    \if\pgf@nfold@prev@visible0%
      \ifpgf@nfold@closejoinsedgecase
        % If the previous segment is a moveto and the current segment is a "close joins" edge case,
        % nothing needs to be drawn here (the relevant draw call will be made at the join of the subsequent
        % segment). We must therefore make sure that we move to the correct end point of this segment.
        % Counterintuitively, this is given by the offset of \pgf@nfold@cur@movedFIRST since the start and end
        % are reversed in the edge case.
        \edef\pgf@nfold@macrotoadd{%
          \noexpand\pgf@nfold@token@edgecase@movetostart{\pgf@nfold@cur@movedfirst}{\pgf@nfold@cur@angle@i}%
        }%
        \pgf@nfold@addmacro\pgf@parsed@cur@conn@seg%
      \fi
    \else
      % If we draw the join when the start angle is close to 180 degrees, we get a division by zero
      \ifpgf@nfold@angletoosharp\else
        \if\pgf@nfold@cur@type z\else
          \pgf@nfold@process@join
        \fi
      \fi
    \fi
    % Step 2.2: Store information that may be needed later
    % Step 2.2.1: Store where the current (non-offset) end point was relocated
    % in order to make space for the end join. This may be used if the next
    % segment begins with a join
    \let\pgf@nfold@prev@segment@end\pgf@nfold@cur@movedlast
    % Step 2.2.2: Store the tangent of the first proper segment of closed path.
    % This is needed in case the \pgfpathclose-segment has length zero,
    % since in that case its tangent cannot be computed.
    \if\pgf@nfold@cur@type i
      \let\pgf@nfold@connsubpath@tang@i\pgf@nfold@next@tang@i%
      \let\pgf@nfold@connsubpath@angle@i\pgf@nfold@next@angle@i%
    \fi
    %
    % Step 3: Draw the new segment.
    %
    % The value of \ifpgf@nfold@continuesegment decides whether we start with a moveto.
    \if\pgf@nfold@cur@type l
      % In the edge case, one join is followed immediately by the next. The line segment
      % thus has a negative length and will be skipped.
      \ifpgf@nfold@closejoinsedgecase\else
        \edef\pgf@nfold@macrotoadd{%
          \expandafter\noexpand\ifpgf@nfold@continuesegment%
            \pgf@nfold@token@lineto@continue%
          \else%
            \pgf@nfold@token@lineto%
          \fi{\pgf@nfold@cur@movedfirst}{\pgf@nfold@cur@movedlast}{\pgf@nfold@cur@tang@i}%
        }%
        \pgf@nfold@addmacro\pgf@parsed@cur@conn@seg%
      \fi
    \fi
    \if\pgf@nfold@cur@type o
      \def\pgf@nfold@macrotoadd{\pgf@nfold@token@closepath}%
      \pgf@nfold@addmacro\pgf@parsed@cur@conn@seg%
    \fi
    \if\pgf@nfold@cur@type z
      % zero and non-zero closepath's differ in the join handling, but are identical in rendering
      \def\pgf@nfold@macrotoadd{\pgf@nfold@token@closepath}%
      \pgf@nfold@addmacro\pgf@parsed@cur@conn@seg%
    \fi
    \if\pgf@nfold@cur@type c
      \ifpgf@nfold@continuesegment
        \pgf@subdividecurve{\pgf@nfold@cur@movedfirst}{\pgf@nfold@cur@supporta}{\pgf@nfold@cur@supportb}{\pgf@nfold@cur@movedlast}{\pgf@offset@max@recursion}{0}{\pgf@nfold@addcurvesegment@callback@continue}
      \else
        \pgf@subdividecurve{\pgf@nfold@cur@movedfirst}{\pgf@nfold@cur@supporta}{\pgf@nfold@cur@supportb}{\pgf@nfold@cur@movedlast}{\pgf@offset@max@recursion}{0}{\pgf@nfold@addcurvesegment@callback}%
      \fi
    \fi
    \if\pgf@nfold@cur@type i
      \edef\pgf@nfold@macrotoadd{%
        \noexpand\pgf@nfold@token@invisibleline{\pgf@nfold@cur@movedfirst}{\pgf@nfold@cur@movedlast}{\pgf@nfold@cur@tang@i}%
      }%
      \pgf@nfold@addmacro\pgf@parsed@cur@conn@seg%
    \fi
    % Step 4: Extend into the arrow tip at the end (if present)
    \if\pgf@nfold@next@type t%
      \ifnum\pgf@nfold@end@arrowcode=1
        \edef\pgf@nfold@macrotoadd{%
          \noexpand\pgf@nfold@extendtotip{e}{\pgf@nfold@cur@last}{\pgf@nfold@cur@angle@ii}}%
        \pgf@nfold@addmacro\pgf@parsed@cur@conn@seg%
      \fi%
    \fi%
  \fi% end if current visible
}


\def\pgf@nfold@addcurvesegment@callback#1#2#3#4#5{%
  \if#50%
    \edef\pgf@nfold@macrotoadd{%
      % The subdivision algorithm has already computed the tangents
      \noexpand\pgf@nfold@token@curveto{#1}{#2}{#3}{#4}{\pgf@tmp@tang@i}{\pgf@tmp@tang@ii}%
    }%
    \pgf@nfold@addmacro\pgf@parsed@cur@conn@seg%
  \else%
    \pgf@nfold@addcurvesegment@callback@continue{#1}{#2}{#3}{#4}{#5}%
  \fi%
}

\def\pgf@nfold@addcurvesegment@callback@continue#1#2#3#4#5{%
  % The subdivision algorithm has already computed the tangents
  \edef\pgf@nfold@macrotoadd{%
    \noexpand\pgf@nfold@token@curveto@continue{#1}{#2}{#3}{#4}{\pgf@tmp@tang@i}{\pgf@tmp@tang@ii}%
  }%
  \pgf@nfold@addmacro\pgf@parsed@cur@conn@seg%
}


% Rendering arrow tips
% --------------------

% Precomputed intersections
%
% For arrows of order n > 2 with an Implies tip, the constituent parts of the n-fold arrow
% end somewhere in the middle of the tip. The exact end point must be computed using
% the intersections library. To speed up compilation times, the intersection points are precomputed
% up to n = 5. If your document contains arrows of order 6 or larger, consider adding those
% as well; the values are output in the log file.
\expandafter\def\csname pgf@nfold@intersec@cache@2@3\endcsname{\pgfqpoint{2pt}{0pt}}
\expandafter\def\csname pgf@nfold@intersec@cache@2@4\endcsname{\pgfqpoint{0.94063pt}{-0.33333pt}}
\expandafter\def\csname pgf@nfold@intersec@cache@3@4\endcsname{\pgfqpoint{0.94063pt}{0.33333pt}}
\expandafter\def\csname pgf@nfold@intersec@cache@2@5\endcsname{\pgfqpoint{0.64167pt}{-0.5pt}}
\expandafter\def\csname pgf@nfold@intersec@cache@3@5\endcsname{\pgfqpoint{2pt}{0pt}}
\expandafter\def\csname pgf@nfold@intersec@cache@4@5\endcsname{\pgfqpoint{0.64167pt}{0.5pt}}
% intersections are precomputed up to this order
\def\pgf@nfold@intersec@numcached{5}

\newif\ifpgf@nfold@ontheedge
% This macro extends the arrow body to the tips
% #1: s=start, e=end
% #2: start/end point of the path
% #3: angle
\def\pgf@nfold@extendtotip#1#2#3{
  \ifpgf@nfold@intersectionsnotloaded
    \pgfutil@packageerror{tikz-nfold}{%
        If `nfold' is larger than \pgf@nfold@intersec@numcached\space and you use
        an `Implies' arrow tip you need to say \string\usetikzlibrary{intersections}}{}
  \else
  \pgf@nfold@ontheedgetrue
  % Do not extend the arrow for index=1 and index=order, it already ends in the right place
  \ifnum\pgf@nfold@index>1\relax\ifnum\pgf@nfold@index<\pgf@nfold@order\relax%
    \pgf@nfold@ontheedgefalse
  \fi\fi
  \ifpgf@nfold@ontheedge%
    % the extension at the start needs a moveto to the correct starting point
    \if#1s
      \pgfpathmoveto{\pgfpointadd{#2}{\pgfpointpolar{#3+90}{\pgf@nfold@shiftamount}}}%
    \fi
  \else
    % Step 1: Find the intersection of the arrow's path with the head
    \ifcsname pgf@nfold@intersec@cache@\the\pgf@nfold@index @\the\pgf@nfold@order\endcsname
      \pgfextract@process\pgf@nfold@arrowintersect
        {\csname pgf@nfold@intersec@cache@\the\pgf@nfold@index @\the\pgf@nfold@order\endcsname}%
    \else
      % the intersection has not been precomputed, thus compute on the fly here
      \pgfintersectionofpaths{
        % specify the tip
        \pgfpathmoveto{\pgfqpoint{-1.4pt}{2.65pt}}
        \pgfpathcurveto{\pgfqpoint{-0.75pt}{1.25pt}}{\pgfqpoint{1pt}{0.05pt}}{\pgfqpoint{2pt}{0pt}}
        \pgfpathcurveto{\pgfqpoint{1pt}{-0.05pt}}{\pgfqpoint{-0.75pt}{-1.25pt}}{\pgfqpoint{-1.4pt}{-2.65pt}}
      }{
        % extend the body to intersect the tip
        \pgfpathmoveto{\pgfqpoint{-3pt}{\pgf@nfold@shift@fraction pt}}
        \pgfpathlineto{\pgfqpoint{3pt}{\pgf@nfold@shift@fraction pt}}
      }
      \ifnum\pgfintersectionsolutions>0
        \pgfextract@process\pgf@nfold@arrowintersect{\pgfpointintersectionsolution{1}}%
        \immediate\write17{tikz-nfold: computed intersection cache@\the\pgf@nfold@index @\the\pgf@nfold@order: \string\pgfqpoint{\the\pgf@x}{\the\pgf@y}^^J}
        % add the new intersection to the cache
        \expandafter\xdef\csname pgf@nfold@intersec@cache@\the\pgf@nfold@index @\the\pgf@nfold@order\endcsname{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}
      \else
        % this is a failsafe and should never be reached
        \pgfutil@packagewarning{tikz-nfold}{did not find intersection}
        \pgfextract@process\pgf@nfold@arrowintersect{\pgfqpoint{0pt}{\pgf@nfold@shift@fraction pt}}%
      \fi
    \fi% if precomputed
    % Step 2: Extend the arrow body to the intersection point.
    % If the tip is at the beginning of the path, we have to move to the intersection
    % and then draw a line to the "regular" starting point. The subsequent segment then
    % should omit its moveto.
    % If the tip is at the end, we are already in the right position and only need to extend
    % the current path to the intersection point.
    \begingroup
      \pgftransformreset
      \pgftransformshift{#2}
      \pgftransformrotate{#3}
      \if#1s
        \pgftransformxscale{-1}
      \fi
      % we don't want to undo the shift by .42\pgflinewidth after the scaling
      \pgfutil@tempdima=\pgf@nfold@hwidth
      \pgfutil@tempdima=\pgf@nfold@shift@fraction\pgfutil@tempdima
      \pgfextract@process\pgf@nfold@startofextension
        {\pgfpointtransformed{\pgfqpoint{0pt}{\pgfutil@tempdima}}}
      % 0.5 - 0.06 = 0.42
      \pgftransformshift{\pgfqpoint{.42\pgflinewidth}{0pt}}
      \pgftransformscale{\pgf@nfold@hwidth}
      \pgfextract@process\pgf@nfold@arrowintersect{\pgfpointtransformed{\pgf@nfold@arrowintersect}}
      \global\let\pgf@nfold@startofextension\pgf@nfold@startofextension
      \global\let\pgf@nfold@arrowintersect\pgf@nfold@arrowintersect
    \endgroup
    \if#1s
      \pgfpathmoveto{\pgf@nfold@arrowintersect}
      % This is precisely the start of the body, shifted vertically
      \pgfpathlineto{\pgf@nfold@startofextension}
    \else\if#1e
      \pgfpathlineto{\pgf@nfold@arrowintersect}
    \else
      \pgfutil@packageerror{tikz-nfold}{Invalid argument to \string\pgf@nfold@extendtotip: \meaning#1}{}
    \fi\fi
    \pgftransformreset
    \fi% if 1 < i < nArrows
  \fi% if intersections is needed and not loaded
}

% Parsing the arrow tips
% ----------------------
%
% We need to detect if the user has set Implies[] arrows at the start and/or end tip.
% To do so, we parse \pgf@start@tip@sequence. If the user specifies Implies[] manually,
% we find that
%   pgf@start@tip@sequence=\pgf@arrow@handle{Implies}{...}
% However, in other cases (like tikz-cd) we may find 
%   \pgf@arrow@handle@shorthand@empty {\csname pgf@ar@means@tikzcd implies cap\endcsname }
% In such cases we must expand the first parameter once and then match as above.

% Set global defaults
\def\pgf@nfold@start@arrowcode{0}
\def\pgf@nfold@end@arrowcode{0}

\def\pgf@nfold@parsearrows{
  \ifpgfutil@tempswa% this is set in \pgfusepath and stores whether we draw arrow tips at all
    \expandafter\pgf@nfold@parsearrowmacro\pgf@start@tip@sequence\relax
    \let\pgf@nfold@start@arrowcode\pgf@nfold@detectedarrow
    \expandafter\pgf@nfold@parsearrowmacro\pgf@end@tip@sequence\relax
    \let\pgf@nfold@end@arrowcode\pgf@nfold@detectedarrow
  \else
    \def\pgf@nfold@start@arrowcode{0}
    \def\pgf@nfold@end@arrowcode{0}
  \fi
}

\def\pgf@nfold@parsearrowmacro#1{%
  \def\pgf@nfold@detectedarrow{0}
  \ifx#1\relax
    \let\pgf@next\relax
  \else
    \ifx#1\pgf@arrow@handle
      % found \pgf@arrow@handle{...}, now parse the first parameter
      \let\pgf@next\pgf@nfold@parse@arrow@handle
    \else
      \ifx#1\pgf@arrow@handle@shorthand@empty
        \let\pgf@next\pgf@nfold@parse@shorthandempty
      \else
        % found nothing
        \let\pgf@next\pgfutil@gobble@until@relax
      \fi
    \fi
  \fi
  \pgf@next
}

\def\pgf@nfold@param@Implies{Implies}

\def\pgf@nfold@parse@arrow@handle#1{%
  \def\pgf@tmp{#1}
  \ifx\pgf@tmp\pgf@nfold@param@Implies
    \def\pgf@nfold@detectedarrow{1}
  \fi
  \pgfutil@gobble@until@relax
}

\def\pgf@nfold@parse@shorthandempty#1{
  % Expand #1 once (\pgf@arrow@handle@shorthand@empty is just an identity operator)
  \expandafter\def\expandafter\pgf@tmp\expandafter{#1}
  \expandafter\pgf@nfold@parsearrowmacro\pgf@tmp\relax
  % still need to gobble the rest of the orginal arrow definition
  \pgfutil@gobble@until@relax
}


%
% Hooking into pgf's rendering pipeline
% -------------------------------------
%
% The new code has to be injected into \pgfusepath (pgfcorepathusage.code.tex). For rendering the new paths,
% \pgf@stroke@inner@line is a natural choice as this is where /tikz/double is rendered. However, we also
% need to disable rendering the ordinary path, which is not as easy. In the future I will make a pull request
% to TikZ to simplify such injections.
%
% The call to draw the path comes right before \pgf@stroke@inner@line. The macro before \pgf@stroke@inner@line
% is either \pgf@path@check@proper or \pgf@prepare@start@of@path (depending on the result of the proper check).
% We therefore must inject code into both of them to see if nfold is enabled. If it is, we call the old macro,
% cache and delete the current softpath (so the call to \pgfsyssoftpath@invokecurrentpath has no effect), then we
% restore and offset the cached softpath in \pgf@stroke@inner@line.
%
% The macros \pgf@path@check@proper and \pgf@prepare@start@of@path are also used in \pgf@up@draw@arrows@only,
% so we must make sure that the latter is unaffected by the modifications. Luckily, this turns out not to be
% a problem - the only macros that are called after the modified ones are \pgf@add@arrow@at@start and
% \pgf@add@arrow@at@end, which do not change their behaviour even if we modify the paths.
%

\newcount\pgf@nfold@order
\pgf@nfold@order=1

\def\pgf@nfold@preparenfoldpath{%
  \ifnum\pgf@nfold@order>1\relax
    \ifdim\pgfinnerlinewidth>0pt\relax
      % Hack the rendering pipeline: There is a \pgfsyssoftpath@invokecurrentpath call following
      % which we do not want if nfold is active. We therefore clear the current path here
      % and then perform the nfold drawing in our modification of \pgf@stroke@inner@line
      \pgfsyssoftpath@getcurrentpath\pgf@nfold@cachedpath%
      \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
    \else
      \pgfutil@packageerror{tikz-nfold}{Must set \string\pgfinnerlinewidth\space to use nfold, e.g. by setting /tikz/double distance}{}
    \fi
  \fi
}

\let\pgf@nfold@old@path@check@proper\pgf@path@check@proper
\def\pgf@path@check@proper{%
  \pgf@nfold@old@path@check@proper%
  \ifpgfutil@tempswa\else%
    % if \pgfutil@tempswa is false, this is the last macro we can overwrite before the draw call.
    % Otherwise, we inject into \pgf@prepare@start@of@path%
    \pgf@nfold@preparenfoldpath%
  \fi%
}

\let\pgf@nfold@old@prepare@start@of@path\pgf@prepare@start@of@path
\def\pgf@prepare@start@of@path{%
  \pgf@nfold@old@prepare@start@of@path%
  \pgf@nfold@preparenfoldpath%
}

\let\pgf@nfold@old@stroke@inner@line\pgf@stroke@inner@line
\def\pgf@stroke@inner@line{%
  \ifnum\pgf@nfold@order>1\relax%
    \pgf@nfold@render@cached@softpath%
  \else%
    % Old behaviour
    \pgf@nfold@old@stroke@inner@line%
  \fi%
}


%
% Parsing the soft path
% ---------------------
%
% Part of the code below is based on pgfmoduledecorations.code.tex (c) 2019 Mark Wibrow and Till Tantau.
% Quite similar to decorations we parse the current soft path and put it into a form that makes it easier
% to iterate over.
%

% The parsing macros below add \pgf@nfold@process@...-macros to \pgf@cur@conn@subpath.
% Once a connected sub-path is parsed, calling \pgf@cur@conn@subpath triggers processing.

\def\pgf@nfold@parsemoveto#1#2{%
  \ifx\pgf@cur@conn@subpath\pgfutil@empty%
    % This case happens for the very first segment or for double movetos.
    % We need special treatment here, as otherwise the arrow tip extension
    % does not work correctly. The \pgf@nfold@processmoveto will be called
    % in \pgf@nfold@process@conn@subpath.
    \def\pgf@nfold@parser@last@moveto{{#1}{#2}}%
    % Make sure \pgf@cur@conn@subpath is no longer empty so double movetos are not
    % treated the same as single movetos. This is also relevant to arrow tip extensions
    \def\pgf@cur@conn@subpath{\relax}%
  \else%
    \def\pgf@nfold@macrotoadd{\pgf@nfold@processmoveto{#1}{#2}}%
    \pgf@nfold@addmacro\pgf@cur@conn@subpath%
    \pgf@nfold@lastconnsubpathfalse%
    % A moveto marks the beginning/end of one connected sub-path
    \pgf@nfold@process@conn@subpath%
    \let\pgf@nfold@last@closepath@from\pgfutil@empty%
    \let\pgf@cur@conn@subpath\pgfutil@empty%
    % set up "first" again which may be needed for the arrow tip extension
    \pgf@nfold@parser@setupfirst%
    \def\pgf@nfold@parser@last@moveto{{#1}{#2}}%
  \fi%
  \pgf@nfold@parsesoftpath@finish{#1}{#2}%
}

\def\pgf@nfold@parselineto#1#2{%
  \def\pgf@nfold@macrotoadd{\pgf@nfold@processlineto{#1}{#2}}%
  \pgf@nfold@addmacro\pgf@cur@conn@subpath%
  \pgf@nfold@parsesoftpath@finish{#1}{#2}%
}

\def\pgf@nfold@parseclosepath#1#2{%
  \let\pgf@nfold@last@closepath@from\pgf@nfold@parser@previous@pt%
  \def\pgf@nfold@macrotoadd{\pgf@nfold@processclosepath{#1}{#2}}%
  \pgf@nfold@addmacro\pgf@cur@conn@subpath%
  \pgf@nfold@parsesoftpath@finish{#1}{#2}%
}

\def\pgf@nfold@parsecurveto#1#2{%
  \edef\pgf@nfold@macrotoadd{\noexpand\pgf@nfold@processcurveto\pgf@nfold@parser@supporta\pgf@nfold@parser@supportb{#1}{#2}}%
  \pgf@nfold@addmacro\pgf@cur@conn@subpath%
  \pgf@nfold@parsesoftpath@finish{#1}{#2}%
}

% Mostly for the sake of completeness; using TikZ' "\path (0,0) rectangle (1,1);" does not call this code
\def\pgf@nfold@parserect#1#2#3#4{%
  \pgf@nfold@parsemoveto{#1}{#2}%
  \pgf@xc=#1\relax
  \pgf@yc=#2\relax
  \pgf@xd=#3\relax
  \pgf@yd=#4\relax
  \advance\pgf@yc\pgf@yd%
  \edef\pgf@temp{{\the\pgf@xc}{\the\pgf@yc}}%
  \expandafter\pgf@nfold@parselineto\pgf@temp%
  \advance\pgf@xc\pgf@xd%
  \edef\pgf@temp{{\the\pgf@xc}{\the\pgf@yc}}%
  \expandafter\pgf@nfold@parselineto\pgf@temp%
  \advance\pgf@yc-\pgf@yd%
  \edef\pgf@temp{{\the\pgf@xc}{\the\pgf@yc}}%
  \expandafter\pgf@nfold@parselineto\pgf@temp%
  \advance\pgf@xc-\pgf@xd%
  \edef\pgf@temp{{\the\pgf@xc}{\the\pgf@yc}}%
  \expandafter\pgf@nfold@parseclosepath\pgf@temp%
  \pgf@nfold@parsemoveto{#1}{#2}%
}

%
% In order to correctly implement \pgfpathclose we already need to know about
% the \pgfpathclose (and the penultimate point) at the beginning of this
% connected sub-path, as these data affect the first/last join.
% We therefore parse one connected sub-path of the softpath and store it in a modified
% form in \pgf@cur@conn@subpath. When reaching the end of the connected sub-path we commence
% the processing to turn \pgf@cur@conn@subpath into a parsed path. We do this for
% all connected sub-paths and concatenate all the parsed paths.
%

\def\pgf@nfold@parsesoftpath#1#2{%
  \let\pgf@cur@conn@subpath\pgfutil@empty%
  \let\pgf@all@parsed@subpaths\pgfutil@empty%
  \edef\pgf@nfold@parser@last@moveto{{\the\pgf@path@lastx}{\the\pgf@path@lasty}}%
  \let\pgf@nfold@last@closepath@from\pgfutil@empty%
  \pgf@nfold@parser@setupfirst%
  \expandafter\pgf@nfold@@parsesoftpath#1\pgf@stop{}{}%
  \let#2\pgf@all@parsed@subpaths%
}%

\def\pgf@nfold@@parsesoftpath#1#2#3{%
  \let\pgf@next\pgf@nfold@@parsesoftpath%
  \ifx#1\pgf@stop%
    \def\pgf@nfold@macrotoadd{\pgf@nfold@processlast}%
    \pgf@nfold@addmacro\pgf@cur@conn@subpath%
    \pgf@nfold@lastconnsubpathtrue%
    \pgf@nfold@process@conn@subpath%
    \let\pgf@next\relax%
  \else%
    \ifx#1\pgfsyssoftpath@movetotoken%
      \pgf@nfold@parsemoveto{#2}{#3}%
    \else%
      \ifx#1\pgfsyssoftpath@linetotoken%
        \pgf@nfold@parselineto{#2}{#3}%
      \else%
        \ifx#1\pgfsyssoftpath@curvetosupportatoken%
          \def\pgf@nfold@parser@supporta{{#2}{#3}}%
        \else%
          \ifx#1\pgfsyssoftpath@curvetosupportbtoken%
            \def\pgf@nfold@parser@supportb{{#2}{#3}}%
          \else%
            \ifx#1\pgfsyssoftpath@curvetotoken%
              \pgf@nfold@parsecurveto{#2}{#3}%
            \else%
              \ifx#1\pgfsyssoftpath@closepathtoken%
                \pgf@nfold@parseclosepath{#2}{#3}%
              \else%
                \ifx#1\pgfsyssoftpath@rectcornertoken%
                  \def\pgf@nfold@parser@rectcorner{{#2}{#3}}%
                \else%
                  \ifx#1\pgfsyssoftpath@rectsizetoken%
                    \expandafter\pgf@nfold@parserect\pgf@nfold@parser@rectcorner{#2}{#3}%
                  \else%
                    \pgfutil@packageerror{tikz-nfold}{Unrecognised soft path token `#1'}{}%
                  \fi%
                \fi%
              \fi%
            \fi%
          \fi%
        \fi%
      \fi%
    \fi%
  \fi%
  % We call \pgf@nfold@parsesoftpath@finish in all parsing macros instead of here because
  % \pgf@nfold@parserect calls other parsing macros internally
  \pgf@next%
}%

\def\pgf@nfold@parsesoftpath@finish#1#2{%
  \def\pgf@nfold@parser@previous@pt{{#1}{#2}}%
  % store the last two segments, as they might be needed for zero-length \pgfpathclose-segments
  \let\pgf@nfold@sectolast@segment\pgf@nfold@last@segment%
  \let\pgf@nfold@last@segment\pgf@nfold@macrotoadd%
}

\def\pgf@nfold@process@conn@subpath{%
  \let\pgf@parsed@cur@conn@seg\pgfutil@empty%
  \ifx\pgf@nfold@last@closepath@from\pgfutil@empty%
    \expandafter\pgf@nfold@processmoveto\pgf@nfold@parser@last@moveto%
  \else%
    % This connected sub-path ends on a closepath. In order to get
    % the join right, we prepend the current sub-path with an invisible line
    % identical to the line of the \pgfpathclose.
    \expandafter\pgf@nfold@processmoveto\pgf@nfold@last@closepath@from%
    \expandafter\pgf@nfold@processinvisibleline\pgf@nfold@parser@last@moveto%
  \fi%
  \pgf@cur@conn@subpath%
  \let\pgf@nfold@macrotoadd\pgf@parsed@cur@conn@seg%
  \pgf@nfold@addmacro\pgf@all@parsed@subpaths%
}

%
% Values for \pgf@nfold@next@type:
% f=first, m=moveto, c=curveto, l=lineto, r=rect, o=closepath, z=zero length closepath, t=last, i=invisibleline
%

\def\pgf@nfold@processmoveto#1#2{%
  \pgf@nfold@process@moveup%
  \let\pgf@nfold@next@type=m%
  \let\pgf@nfold@next@visible=0%
  \edef\pgf@nfold@next@last{\pgf@x#1\pgf@y#2}%
  \pgf@nfold@process@segment%
}%

% Common code for processlineto and processclosepath
\def\pgf@nfold@process@line@common#1#2#3{%
  \pgf@nfold@process@moveup%
  \pgfextract@process\pgf@tmp@tang@i{\pgfpointnormalised{}\global\let\pgf@nfold@tmp\pgf@tmp}
  \let\pgf@nfold@next@type=#3%
  \let\pgf@nfold@next@visible=1%
  \let\pgf@nfold@next@tang@i\pgf@tmp@tang@i
  \let\pgf@nfold@next@tang@ii\pgf@tmp@tang@i
  \let\pgf@nfold@next@angle@i\pgf@nfold@tmp
  \let\pgf@nfold@next@angle@ii\pgf@nfold@tmp
  \let\pgf@nfold@next@first\pgf@nfold@cur@last
  \def\pgf@nfold@next@last{\pgf@x#1\pgf@y#2}%
  \pgf@nfold@process@segment%
}

\def\pgf@nfold@processlineto#1#2{%
  % the current end is still stored in next@last because process@moveup has not been called yet
  \pgf@process{\pgfpointdiff{\pgf@nfold@next@last}{\pgf@x#1\pgf@y#2}}%
  \pgfpointtaxicabnorm\pgf@xa%
  % remove degenerate line segments (reduces glitches)
  \ifdim\pgf@xa>.1pt\relax%
    \pgf@nfold@process@line@common{#1}{#2}{l}%
  \fi%
}%

\def\pgf@nfold@processcurveto#1#2#3#4#5#6{%
  \pgf@nfold@process@moveup%
  \pgf@offset@compute@tangents{\pgf@nfold@cur@last}{\pgf@x#1\pgf@y#2}{\pgf@x#3\pgf@y#4}{\pgf@x#5\pgf@y#6}%
  \let\pgf@nfold@next@type=c%
  \let\pgf@nfold@next@visible=1%
  % the following only need to be set if visible=1
  \let\pgf@nfold@next@tang@i=\pgf@tmp@tang@i
  \let\pgf@nfold@next@tang@ii=\pgf@tmp@tang@ii
  \let\pgf@nfold@next@angle@i\pgf@tmp@angle@i
  \let\pgf@nfold@next@angle@ii\pgf@tmp@angle@ii
  \let\pgf@nfold@next@first\pgf@nfold@cur@last
  \def\pgf@nfold@next@supporta{\pgf@x#1\pgf@y#2}
  \def\pgf@nfold@next@supportb{\pgf@x#3\pgf@y#4}
  \def\pgf@nfold@next@last{\pgf@x#5\pgf@y#6}
  \pgf@nfold@process@segment%
}%

\def\pgf@nfold@processclosepath#1#2{%
  \pgf@process{\pgfpointdiff{\pgf@nfold@next@last}{\pgf@x#1\pgf@y#2}}%
  % closepath segments should always be processed even if they have zero length
  \pgfpointtaxicabnorm\pgf@xa%
  \ifdim\pgf@xa<0.1pt\relax%
    \pgf@nfold@process@closepath@zerolength{#1}{#2}%
  \else%
    \pgf@nfold@process@line@common{#1}{#2}{o}%
  \fi%
}%

\def\pgf@nfold@process@closepath@zerolength#1#2{%
  \pgf@nfold@process@moveup%
  \let\pgf@nfold@next@type=z%
  \let\pgf@nfold@next@visible=1%
  % Set the start and end tangent to the tangent of the first segment
  \let\pgf@nfold@next@tang@i\pgf@nfold@connsubpath@tang@i
  \let\pgf@nfold@next@tang@ii\pgf@nfold@connsubpath@tang@i
  \let\pgf@nfold@next@angle@i\pgf@nfold@connsubpath@angle@i
  \let\pgf@nfold@next@angle@ii\pgf@nfold@connsubpath@angle@i
  \let\pgf@nfold@next@first\pgf@nfold@cur@last
  % If problems arise, we need to put a fake point here (like \pgf@nfold@next@first + \pgf@nfold@next@tang@i)
  \def\pgf@nfold@next@last{\pgf@x#1\pgf@y#2}%
  \pgf@nfold@process@segment%
}

\def\pgf@nfold@processinvisibleline#1#2{%
  \pgf@process{\pgfpointdiff{\pgf@nfold@next@last}{\pgf@x#1\pgf@y#2}}%
  \pgfpointtaxicabnorm\pgf@xa%
  % In order to correctly render the start/end join in a closed path,
  % the \pgfpathclose segment is copied to the start of the path as an invisible line.
  % Counterintuitively, an "invisibleline" segment has next@visible=1 because
  % we want its end join to be rendered.
  % In case the \pgfpathclose segment has non-zero length, we can just use a copy of
  % this segment for the invisible line. Otherwise, the invisble line segment must will receive
  % the same angle/tangent as the last finite-sized segment, which is the second-to-last
  % segment overall (cached in \pgf@nfold@sectolast@segment).
  \ifdim\pgf@xa>.1pt\relax%
    \pgf@nfold@process@line@common{#1}{#2}{i}%
  \else%
    \begingroup%
      % find the tangent of the second-to-last segment
      \let\pgf@nfold@process@segment\relax%
      \pgf@nfold@sectolast@segment%
      \global\let\pgf@nfold@tmp\pgf@nfold@next@tang@ii%
    \endgroup%
    % Construct an invisible line with length 1pt and the correct tangent.
    % This step might not be needed since the join computations only require the tangent,
    % but the invisibleline segment would be inconsistent otherwise, so better play it safe.
    \pgfextract@process\pgf@nfold@next@first{\pgfpointdiff{\pgf@nfold@tmp}{\pgfqpoint{#1}{#2}}}%
    % write the tangent into (\pgf@x, \pgf@y) where the next macro expects it to be
    \pgf@nfold@tmp%
    \pgf@nfold@process@line@common{#1}{#2}{i}%
  \fi%
}%

\def\pgf@nfold@processlast{%
  \pgf@nfold@process@moveup%
  \let\pgf@nfold@next@type=t%
  \let\pgf@nfold@next@visible=0%
  \pgf@nfold@process@segment%
}

% adds the contents of \pgf@nfold@macrotoadd to #1
\def\pgf@nfold@addmacro#1{%
  % need a \gdef because we have nested groups in the subdivision
  \expandafter\expandafter\expandafter\gdef%
  \expandafter\expandafter\expandafter#1%
  \expandafter\expandafter\expandafter{%
  \expandafter#1\pgf@nfold@macrotoadd}%
}


%
% Tokens for the parsed and processed path
% ----------------------------------------
%

%#3: cached normalised tangent (for efficiency)
\def\pgf@nfold@token@lineto#1#2#3{%
  \pgfoffsetline@{#1}{#2}{\pgf@nfold@shiftamount}{#3}%
}

\def\pgf@nfold@token@lineto@continue#1#2#3{%
  \pgfoffsetlinenomove@{#1}{#2}{\pgf@nfold@shiftamount}{#3}%
}

\def\pgf@nfold@token@invisibleline#1#2#3{%
  % An invisible line should execute a moveto to the end point of the line
  \pgfqpointscale{\pgf@nfold@shiftamount}{#3}%
  \pgf@xc=-\pgf@y%
  \pgf@y=\pgf@x%
  \pgf@x=\pgf@xc%
  \pgfpathmoveto{\pgfpointadd{}{#2}}%
}

% #5, #6: cached normalised tangents at start and end (for efficiency)
\def\pgf@nfold@token@curveto#1#2#3#4#5#6{%
  \def\pgf@tmp@tang@i{#5}%
  \def\pgf@tmp@tang@ii{#6}%
  \pgf@offset@bezier@segment@{#1}{#2}{#3}{#4}{\pgf@nfold@shiftamount}%
  \pgfpathmoveto{\pgf@bezier@offset@i}%
  \pgfpathcurveto{\pgf@bezier@offset@ii}{\pgf@bezier@offset@iii}{\pgf@bezier@offset@iv}%
}

\def\pgf@nfold@token@curveto@continue#1#2#3#4#5#6{%
  \def\pgf@tmp@tang@i{#5}%
  \def\pgf@tmp@tang@ii{#6}%
  \pgf@offset@bezier@segment@{#1}{#2}{#3}{#4}{\pgf@nfold@shiftamount}%
  \pgfpathcurveto{\pgf@bezier@offset@ii}{\pgf@bezier@offset@iii}{\pgf@bezier@offset@iv}%
}

\def\pgf@nfold@token@closepath{%
  \pgfpathclose%
}

% This is needed for some edge case explained above.
% #1: segment@start, which is actually the end point of the current segment in the edge case
% #2: the angle of the current segment (start or end does not matter for straight lines)
\def\pgf@nfold@token@edgecase@movetostart#1#2{%
  \pgfpathmoveto{\pgfpointadd%
    {#1}{\pgfpointpolar{#2+90}{\pgf@nfold@shiftamount}}}%
}


\def\pgf@nfold@parser@setupfirst{%
  \let\pgf@nfold@next@type=f%
  % technically, @visible can be derived from @type, but I think this is more efficient
  \let\pgf@nfold@next@visible=0%
  \edef\pgf@nfold@next@last{\pgf@x\the\pgf@path@lastx\pgf@y\the\pgf@path@lasty}%
  % We do not set any of the other macros like \pgf@nfold@next@tang@i or \pgf@nfold@next@first;
  % any attempt to read them implies that there is a bug elsewhere, so crashing is desired.
}

\def\pgf@nfold@clampangle{
  % The computed angles are values between 0 and 360, so their difference is between 360 and -360;
  % we want the difference to be between -180 and 180
  \ifdim\pgfmathresult pt<-180pt\relax
    \pgfutil@tempdima=\pgfmathresult pt
    \advance\pgfutil@tempdima by 360pt
    \edef\pgfmathresult{\pgf@sys@tonumber\pgfutil@tempdima}
  \else\ifdim\pgfmathresult pt>180pt\relax
    \pgfutil@tempdima=\pgfmathresult pt
    \advance\pgfutil@tempdima by -360pt
    \edef\pgfmathresult{\pgf@sys@tonumber\pgfutil@tempdima}
  \fi\fi
}


\def\pgf@nfold@process@moveup{%
  \let\pgf@nfold@prev@type\pgf@nfold@cur@type%
  \let\pgf@nfold@prev@visible\pgf@nfold@cur@visible%
  \let\pgf@nfold@prev@tang@i\pgf@nfold@cur@tang@i%
  \let\pgf@nfold@prev@tang@ii\pgf@nfold@cur@tang@ii%
  \let\pgf@nfold@prev@angle@i\pgf@nfold@cur@angle@i%
  \let\pgf@nfold@prev@angle@ii\pgf@nfold@cur@angle@ii%
  \let\pgf@nfold@prev@first\pgf@nfold@cur@first%
  \let\pgf@nfold@prev@supporta\pgf@nfold@cur@supporta%
  \let\pgf@nfold@prev@supportb\pgf@nfold@cur@supportb%
  \let\pgf@nfold@prev@last\pgf@nfold@cur@last%
  \let\pgf@nfold@cur@type\pgf@nfold@next@type%
  \let\pgf@nfold@cur@visible\pgf@nfold@next@visible%
  \let\pgf@nfold@cur@tang@i\pgf@nfold@next@tang@i%
  \let\pgf@nfold@cur@tang@ii\pgf@nfold@next@tang@ii%
  \let\pgf@nfold@cur@angle@i\pgf@nfold@next@angle@i%
  \let\pgf@nfold@cur@angle@ii\pgf@nfold@next@angle@ii
  \let\pgf@nfold@cur@first\pgf@nfold@next@first%
  \let\pgf@nfold@cur@supporta\pgf@nfold@next@supporta%
  \let\pgf@nfold@cur@supportb\pgf@nfold@next@supportb%
  \let\pgf@nfold@cur@last\pgf@nfold@next@last%
}

%
% user interface
% --------------
%

% Outputs a provided soft path in #1 offset by a distance provided in #2.
\def\pgfoffsetpath#1#2{%
  \begingroup
    \pgfmathsetlengthmacro\pgf@nfold@parsed@hwidth{#2}
    % \pgf@nfold@hwidth must always be positive
    \pgf@x=\pgf@nfold@parsed@hwidth\relax
    \ifdim\pgf@x<0pt\relax
      \pgf@x=-\pgf@x
      \def\pgf@nfold@shift@fraction{-1}
    \else
      \def\pgf@nfold@shift@fraction{1}
    \fi
    \edef\pgf@nfold@parsed@hwidth{\the\pgf@x}
    \pgfoffsetpathqfraction{#1}{\pgf@nfold@parsed@hwidth}{\pgf@nfold@shift@fraction}
  \endgroup
}

% Outputs a provided soft path in #1 offset by #3*#2 where #2 is a length (>= 0 pt)
% and #3 is a number between -1.0 and 1.0. This differs from \pgfoffsetpath{#1}{#2*#3} 
% in how the joins between segments are rendered.  In particular, \pgfoffsetpathfraction{#1}{10pt}{0}
% does *not* yield the original path, but a new path in the centre of #1 drawn at line width 20pt.
%
\def\pgfoffsetpathfraction#1#2#3{%
  \begingroup
    \pgfmathsetlengthmacro\pgf@nfold@parsed@hwidth{#2}
    \pgfmathsetmacro\pgf@nfold@shift@fraction{#3}
    \pgfoffsetpathqfraction{#1}{\pgf@nfold@parsed@hwidth}{\pgf@nfold@shift@fraction}
  \endgroup
}

% This has the same output as the #3-th segment of nfold=#4.
\def\pgfoffsetpathindex#1#2#3#4{%
  \begingroup
    \pgfmathsetmacro\pgf@nfold@shift@fraction{-1+2*(#3-1)/(#4-1)}
    \pgfoffsetpathqfraction{#1}{#2}{\pgf@nfold@shift@fraction}
  \endgroup
}

% A quick version that skips processing the input values
\def\pgfoffsetpathqfraction#1#2#3{%
  \begingroup
    \pgf@x=#2\relax
    \edef\pgf@nfold@hwidth{\the\pgf@x}
    \edef\pgf@nfold@shift@fraction{#3}
    \pgf@x=\pgf@nfold@shift@fraction\pgf@x\relax
    \edef\pgf@nfold@shiftamount{\pgf@sys@tonumber\pgf@x}
    \pgfprocessround{#1}{\pgf@nfold@cachedpath}% remove tokens from the soft path
    \pgf@nfold@parsesoftpath{\pgf@nfold@cachedpath}{\parsedpath}%
  % Transformations are already baked into the path; without this call, they would be applied twice
    \pgftransformreset%
    \parsedpath%
  \endgroup
}

\endinput


==> tikzlibrarynfold.code.tex <==
%% tikzlibrarynfold.code.tex
%% Copyright 2023 Jonathan Schulz
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3c
% of this license or (at your option) any later version.
% The latest version of this license is in
% http://www.latex-project.org/lppl.txt
% and version 1.3c or later is part of all distributions of LaTeX
% version 2008-05-04 or later.
%
% This work has the LPPL maintenance status 'maintained'.
%
% The Current Maintainer of this work is Jonathan Schulz.
%
% This work consists of the files pgflibrarybezieroffset.code.tex,
% tikzlibrarynfold.code.tex, tikz-nfold-doc.tex, and tikz-nfold-doc.pdf.

% TODO update header with list of files
% TODO does the head detection work without arrows.meta?

\usepgflibrary{nfold}
\usetikzlibrary{arrows.meta}

% use \tikzset for scoping reasons, does not appear to be equivalent to \pgfset{/tikz/...=...}
\tikzset{
  nfold/.code={
    \edef\pgf@tmp{\noexpand\pgfkeys{/pgf/nfold=#1}}
    % patch \tikz@double@setup to set /pgf/nfold=#1 as well
    \expandafter\expandafter\expandafter\def%
      \expandafter\expandafter\expandafter\tikz@double@setup%
      \expandafter\expandafter\expandafter{\expandafter\tikz@double@setup\pgf@tmp}
  },
  nfold/.default=2,
  scaling nfold/.code={%
    \pgfscope% scope to contain \tikz@double@setup
      \tikz@double@setup
      % extract double distance between line centers into \pgf@x
      \pgf@nfold@compute@widths@from@double
      \pgf@y=2\pgf@y
      % store (order-1)*\pgf@x in \pgf@xa
      \c@pgf@counta=#1
      \advance\c@pgf@counta by -1\relax
      \global\pgf@y=\c@pgf@counta\pgf@y
    \endpgfscope
    \tikzset{
      double distance between line centers=\pgf@y,
      nfold=#1
    }
  },
  scaling nfold/.default=2,
  % This simply defines the key if tikzcd is not loaded, so we don't run into any errors
  commutative diagrams/scaling nfold/.code={
    \pgfscope% scope to contain \tikz@double@setup
      \tikz@double@setup
      % extract double distance between line centers into \pgf@x
      \pgf@nfold@compute@widths@from@double
      % store (order-1)*\pgf@y in \pgf@ya
      \c@pgf@counta=#1
      \advance\c@pgf@counta by -1\relax
      \pgf@ya=\c@pgf@counta\pgf@y
      % compute the label offset, which is (order-2)*\pgf@y + .5*\pgf@x
      \advance\c@pgf@counta by -1\relax
      \pgf@xa=\c@pgf@counta\pgf@y
      \advance\pgf@xa by .5\pgf@x
      % save the results in \pgf@x and \pgf@y
      \global\pgf@x=\pgf@xa
      \global\pgf@y=2\pgf@ya
    \endpgfscope
    \tikzset{
      commutative diagrams/every label/.append style/.expanded={outer sep=\the\pgf@x},
      double distance between line centers=\pgf@y,
      nfold=#1
    }
  },
  commutative diagrams/scaling nfold/.default=2
}

\endinput
